FLiER: Practical Topology Update Detection Using Sparse PMUs

In this paper, we present a Fingerprint Linear Estimation Routine (FLiER) to identify topology changes in power networks using readings from sparsely-deployed phasor measurement units (PMUs). When a power line, load, or generator trips in a network, or when a substation is reconfigured, the event leaves a unique "voltage fingerprint" of bus voltage changes that we can identify using only the portion of the network directly observed by the PMUs. The naive brute-force approach to identify a failed line from such voltage fingerprints, though simple and accurate, is slow. We derive an approximate algorithm based on a local linearization and a novel filtering approach that is faster and only slightly less accurate. We present experimental results using the IEEE 57-bus, IEEE 118-bus, and Polish 1999-2000 winter peak networks.

==> common.tex <==
\usepackage{amsmath, amssymb, amsthm}
\usepackage{graphicx} 
\usepackage{url}
\usepackage{algpseudocode} 
\usepackage{algorithm}
\usepackage{tikz}
\newcommand{\small}[1]{#1}


==> variations.tex <==
\section{Variations}

FLiER can be modified to handle several variations on the scenarios described 
above.

\begin{enumerate}

\item Multiple topology changes could occur between state estimates.
  In this case, the events will almost never occur simultaneously, but
  will happen some time apart from each other. Because PMUs provide
  real-time readings, we can obtain fingerprints after each event.
  This allows us to convert the problem of identifying multiple
  coincident topology changes into one of identifying a sequence of
  single topology changes, which is a much easier problem to solve.

\item There might be an infeasibly large number of possibilities for
  FLiER to check. This could occur, for example, if there are a large
  number of possible reconfigurations for each substation in a
  network, or if multiple topology changes occur so close together
  that the PMUs can't obtain reliable fingerprint readings between
  events.

This problem can be mitigated by using $L \geq 1$ stages of
\emph{coarse} filtering. In stage $\ell$, a filtering subspace
$\bar{E} A^{-1} U$ is the sum of multiple stage-$\ell+1$ filtering
subspaces. Then the filtering subspaces associated with multiple
distinct events are all contained within a single subspace. This
allows us to ask, ``do \emph{any} of these contingencies seem
likely?'' with a single computation.  The result is a hierarchy of
filtering subspaces where
$$
\tau_i^1 \leq \cdots \leq \tau_i^L \leq \tau_i \leq t_i.
$$

\item The network operator may have knowledge about changes to power
  injections around the network that have occurred since the last
  state estimate; for example, a generator may have tripped
  offline. This can be handled by simply adjusting the right-hand
  sides in Equations \eqref{eq:bus-merge-lin-system},
  \eqref{eq:bus-split-lin-system}, and
  \eqref{eq:line-fail-lin-system1} to include the change in power
  injection.

\item If a network has a large number of PMUs, then the filtering step
  described in Section \ref{sec:filtering}, while much faster than not
  filtering, might still be slower than desirable. In this case, a
  multistage filtering procedure, different from the one described
  above, can be employed. If $m' < m$ and the matrix $R \in
  \mathbb{R}^{m' \times m}$ has orthonormal rows, then $R$ represents
  an orthogonal projection onto a subspace of dimension $m'$.

So, choose a series of random matrices $R_1, ..., R_L$, such that
$R_\ell \in \mathbb{R}^{m_\ell \times m_{\ell+1}}, m_\ell <
m_{\ell+1}$, and precompute the matrices
$$
R_L E A^{-1}, \; R_{L-1} R_L E A^{-1}, \cdots, \left(\prod_{\ell=1}^L R_\ell \right) E A^{-1}.
$$
Then each such matrix can be used to compute a filter score
$\tau^\ell$, as in Equation \eqref{eq:filter}, and
$$
\tau^1_i \leq \cdots \leq \tau^L_i \leq \tau_i \leq t_i.
$$

\end{enumerate}

